SysCaps: Language Interfaces for Simulation Surrogates of Complex Systems

Surrogate models are used to predict the behavior of complex energy systems that are too expensive to simulate with traditional numerical methods. Our work introduces the use of language descriptions, which we call ``system captions'' or SysCaps, to interface with such surrogates. We argue that interacting with surrogates through text, particularly natural language, makes these models more accessible for both experts and non-experts. We introduce a lightweight multimodal text and timeseries regression model and a training pipeline that uses large language models (LLMs) to synthesize high-quality captions from simulation metadata. Our experiments on two real-world simulators of buildings and wind farms show that our SysCaps-augmented surrogates have better accuracy on held-out systems than traditional methods while enjoying new generalization abilities, such as handling semantically related descriptions of the same test system. Additional experiments also highlight the potential of SysCaps to unlock language-driven design space exploration and to regularize training through prompt augmentation.

==> tables/caption_length.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\caption{\textbf{Caption length}. per-building-hourly.}
\label{tab:caption_length}
\begin{tabular}{@{}lc@{}}
\toprule
SimCap length & NRMSE \\ \midrule
Short         & 0.57{\tiny{$\pm$ 0.02}}              \\
Medium        &  0.53{\tiny{$\pm$ 0.01}}            \\
Long          & 0.64{\tiny{$\pm$ 0.02}}          
\end{tabular}
\end{table}

==> tables/floris_hyperparams.tex <==
\begin{table}[t]
\caption{Hyperparameter sweep information.}
\label{tab:grid-search}
\centering
\small
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Model}                               & \textbf{Hyperparameter}     & \textbf{Grid search space}          & \textbf{Best values} \\ \midrule
\multirow{5}{*}{LightGBM}                     & Learning rate                            & From 0.01 to 0.1                            & 0.066                                 \\
                                              & Number of leaves                         & From 40 to 150                              & 149                                   \\
                                              & Subsample                                & From 0.05 to 1.0                            & 0.178                                 \\
                                              & Feature fraction                         & From 0.05 to 1.0                            & 0.860                                 \\
                                              & Min number of data in one leaf           & From 1 to 100                               & 12                                    \\ \midrule
\multirow{4}{*}{ResNet (one-hot)}             & Hidden layers size                & 256, 1024, 2048                       & 1024     \\
                                    & Number of layers                & 2, 8                      &        2             \\
                                    & Batch size                & 128, 256, 512                       &    512                   \\
                                    & Learning rate                & 0.0001, 0.0003, 0.001                       &   0.001                    \\ \midrule
\multirow{4}{*}{ResNet (text)}             & Hidden layers size                & 256, 1024, 2048                       &   256   \\
                                    & Number of layers                & 2, 8                      &        8               \\
                                    & Batch size                & 128, 256, 512                       &    256                   \\
                                    & Learning rate                & 0.0001, 0.0003, 0.001                       &   0.0003                    \\ \midrule                                    
\multirow{5}{*}{Bidirectional LSTM (one-hot)}  & [Hidden layer size, Batch size] & [128, 64], [512, 32], [1024, 32]              & [128, 64]     \\
                                    & Number of layers   & 1, 3, 4, 6, 8                    &      4                 \\
                                    & MLP dimension      & 256                        &  256                     \\
                                    & Learning rate      & {0.00001}, 0.0003, 0.001 & 0.001                      \\ \midrule
\multirow{5}{*}{Bidirectional LSTM (text)}  & [Hidden layer size, Batch size] & [128, 64], [512, 32], [1024, 32]              & [512, 32]     \\
                                    & Number of layers   & 1, 3, 4, 6, 8                    &      1                \\
                                    & MLP dimension      & 256                        &  256                     \\
                                    & Learning rate      & {0.00001}, 0.0003, 0.001 & 0.0003                        \\ \midrule                                    
\multirow{5}{*}{Bidirectional S4 (one-hot)}  & [Hidden layer size, Num. layers]              &     [64,8]  , [128,4]                     & [128,4]     \\
                                    & MLP dimension               & 256                       &      256                 \\
                                    & Batch size              & 32, 64                        &        64               \\
                                    & Learning rate               &   1e-5, 3e-4, 1e-3                     &        3e-4               \\  \midrule 

\multirow{5}{*}{Bidirectional S4 (text)}   & [Hidden layer size, Num. layers]              &     [64,8]  , [128,4]                     & [128, 4]     \\
                                    & MLP dimension               & 256                       &      256                 \\
                                    & Batch size              & 32, 64                        &        32               \\
                                    & Learning rate               &   1e-5, 3e-4, 1e-3                     &        3e-4               \\                                    
                                    \bottomrule
\end{tabular}
\end{table}
